Influencing Incidental Human-Robot Encounters: Expressive movement improves pedestrians' impressions of a quadruped service robot

A single mobile service robot may generate hundreds of encounters with pedestrians, yet there is little published data on the factors influencing these incidental human-robot encounters. We report the results of a between-subjects experiment (n=222) testing the impact of robot body language, defined as non-functional modifications to robot movement, upon incidental pedestrian encounters with a quadruped service robot in a real-world setting. We find that canine-inspired body language had a positive influence on participants' perceptions of the robot compared to the robot's stock movement. This effect was visible across all questions of a questionnaire on the perceptions of robots (Godspeed). We argue that body language is a promising and practical design space for improving pedestrian encounters with service robots.

==> figures/body_movement_table.tex <==
\begin{table*}[tb]
\centering
\resizebox{\widthmodifier\textwidth}{!}{%
\setlength\extrarowheight{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Body Movement} & \textbf{Roll ($rad$)} & \textbf{Pitch ($rad$)} & \textbf{Yaw ($rad$)} & \textbf{Velocity$_x$}(m/s) & \textbf{Rotation Angle ($rad$)} \\ \hline
Wagging           & -$\pi$/16 to $\pi$/16  & 0 & -$\pi$/8 to $\pi$/8            & 0                        & 0                             \\ \hline
Play Bow               & 0             & 0 to 3$\pi$/14     & 0            & 0                        & 0                               \\ \hline
Sit                    & 0             & -$\pi$/7 to 0      & 0            & 0                        & 0                               \\ \hline
Walk in Circle         & 0             & 0              & 0            & 2                        & -1.5 to 1.5                                 \\ \hline
Spin                   & 0             & 0              & 0            & 0                        & -1\ to 1                                  \\ \hline
\end{tabular}
}
\caption{Specifications of the behavioral components of the canine-inspired Body Language Vignette. %developed in response to our elicitation survey results.% Each behavior is specified as a simple motion smoothly interpolating between fixed poses of the robot's torso or walking trajectories, making it implementable on any platform with sufficient range of motion.
\label{rangeTable}}
\end{table*}

==> figures/nonSigTable.tex <==

\begin{table}[]
\centering
\resizebox{6cm}{!} {%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Survey Question} & \textbf{F-Score} & \textbf{P-Value} \\ \hline
Resemblance to a dog     & 1.283            & 0.259            \\ \hline
Natural                  & 0.233            & 0.630            \\ \hline
Lifelike                 & 2.636            & 0.106            \\ \hline
Moving elegantly         & 1.019            & 0.314            \\ \hline
Interactive              & 3.699            & 0.056            \\ \hline
Competent                & 0.099            & 0.754            \\ \hline
Knowledgeable             & 0.194            & 0.660            \\ \hline
Dislike vs. Like         & 0.201            & 0.655            \\ \hline
Pleasant                 & 2.103            & 0.148            \\ \hline
Awful vs. Nice           & 0.907            & 0.342            \\ \hline
Safe                     & 1.151            & 0.285            \\ \hline
Too far                  & 2.758            & 0.098            \\ \hline
Too fast                 & 0.091            & 0.764            \\ \hline
I'm curious              & 0.015            & 0.901            \\ \hline
I'm cautious             & 0.811            & 0.369            \\ \hline
I'm calm                 & 0.248            & 0.619            \\ \hline
I'm nervous              & 0.768            & 0.382            \\ \hline
I'm excited              & 0.098            & 0.755            \\ \hline
I'm scared               & 0.354            & 0.552            \\ \hline
In a classroom           & 1.280            & 0.259            \\ \hline
In a library             & 0.443            & 0.506            \\ \hline
Delivery on campus       & 1.950            & 0.164            \\ \hline
Delivery to home         & 3.186            & 0.076            \\ \hline
Serve at a restaurant    & 2.350            & 0.127            \\ \hline
\end{tabular}
}
\caption{Non-Statistically Significant Survey Results}
\label{table:3}
\end{table}


==> figures/significantTable.tex <==
\begin{table}[]
\centering
\resizebox{6cm}{!} {%
\begin{tabular}{|c|c|c|}
\hline
\textbf{Survey Question} & \textbf{F-Score} & \textbf{P-Value} \\ \hline
Doglike                  & 5.628            & 0.019            \\ \hline
Conscious                & 4.057            & 0.045            \\ \hline
Responsive               & 6.581            & 0.011            \\ \hline
Friendly                 & 11.685           & \textless{}0.001 \\ \hline
Remote-controlled        & 4.727            & 0.031            \\ \hline
Erratic                  & 11.261           & \textless{}0.001 \\ \hline
\end{tabular}
}
\caption{Statistically Significant Survey Results}
\label{table:2}
\end{table}

==> figures/teaser.tex <==
\begin{teaserfigure}
  \includegraphics[width=\textwidth]{images/tailWagging}
  \caption{Stills of a quadruped service robot displaying body language behavior implemented for this study.}
  \Description{The Boston Dynamics Spot as configured for this study. Two stills of the left and right extremes of the tail wagging behavior are shown, with the Spot leaning in opposite directions.}
  \label{fig:teaser}
\end{teaserfigure}
